Toward gas exhaustion in the W51 high-mass protoclusters

We present new JVLA observations of the high-mass cluster-forming region W51A from 2 to 16 GHz with resolution ${\theta}_{fwhm} \approx$ 0.3 - 0.5". The data reveal a wealth of observational results: (1) Currently-forming, very massive (proto-O) stars are traced by o-H2CO $2_{1,1}-2_{1,2}$ emission, suggesting that this line can be used efficiently as a massive protostar tracer. (2) There is a spatially distributed population of $\sim$mJy continuum sources, including hypercompact H ii regions and candidate colliding wind binaries, in and around the W51 proto-clusters. (3) There are two clearly detected protoclusters, W51e and W51 IRS2, that are gas-rich but may have most of their mass in stars within their inner $\sim$ 0.05 pc. The majority of the bolometric luminosity in W51 most likely comes from a third population of OB stars between these clusters. The presence of a substantial population of exposed O-stars coincident with a population of still-forming massive stars, along with a direct measurement of the low mass loss rate via ionized gas outflow from W51 IRS2, together imply that feedback is ineffective at halting star formation in massive protoclusters. Instead, feedback may shut off the large-scale accretion of diffuse gas onto the W51 protoclusters, implying that they are evolving towards a state of gas exhaustion rather than gas expulsion. Recent theoretical models predict gas exhaustion to be a necessary step in the formation of gravitationally bound stellar clusters, and our results provide an observational validation of this process.

==> aamacros.tex <==
\newcommand\arcdeg{\mbox{$^\circ$}\xspace} 

